Virtual memory for real-time systems using hPMP

To satisfy automotive safety and security requirements, memory protection mechanisms are an essential component of automotive microcontrollers. In today's available systems, either a fully physical address-based protection is implemented utilizing a memory protection unit, or a memory management unit takes care of memory protection while also mapping virtual addresses to physical addresses. The possibility to develop software using a large virtual address space, which is agnostic to the underlying physical address space, allows for easier software development and integration, especially in the context of virtualization. In this work, we showcase an extension to the current RISC-V SPMP proposal that enables address redirection for selected address regions, while maintaining the fully deterministic behavior of a memory protection unit.

==> tables/hpmp_config_zero.tex <==
\def\hexaddress(#1){\texttt{0x#1}}

\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Name & Size [KB] & hPMP address A & hPMP cfg A & hPMP address B & hPMP cfg B & hPMP offset B \\\hline
Stack HV & 2 & \hexaddress(2000 0000) & OFF & \hexaddress(2000 07FF) & S TOR RW & \hexaddress(0000 0000) \\\hline
Code HV & 256 & \hexaddress(8000 0000) & OFF & \hexaddress(8003 FFFF) & S TOR RX & \hexaddress(0000 0000) \\\hline
Data HV & 96 & \hexaddress(9080 0000) & OFF & \hexaddress(9081 7FFF) & S TOR RW & \hexaddress(0000 0000) \\\hline\hline

Stack VM1 & 4 & \hexaddress(0000 0000) & OFF & \hexaddress(0000 0FFF) & - TOR RW & \hexaddress(2000 0800) \\\hline
Code VM1 & 512 & \hexaddress(0004 0000) & OFF & \hexaddress(000B FFFF) & - TOR RX & \hexaddress(8000 0000) \\\hline
Data VM1 & 128 & \hexaddress(0100 0000) & OFF & \hexaddress(0101 FFFF) & - TOR RW & \hexaddress(8F00 0000) \\\hline
Data VM1 & 256 & \hexaddress(0102 0000) & OFF & \hexaddress(0103 FFFF) & - TOR RW & \hexaddress(8F7F 8000) \\\hline\hline

Stack VM2 & 4 & \hexaddress(0000 0000) & OFF & \hexaddress(0000 0FFF) & - TOR RW & \hexaddress(2000 1800) \\\hline
Code VM2 & 512 & \hexaddress(0004 0000) & OFF & \hexaddress(0013 FFFF) & - TOR RX & \hexaddress(8008 0000) \\\hline
Data VM2 & 128 & \hexaddress(0100 0000) & OFF & \hexaddress(0101 FFFF) & - TOR RW & \hexaddress(8F02 0000) \\\hline
Data VM2 & 256 & \hexaddress(0102 0000) & OFF & \hexaddress(0105 FFFF) & - TOR RW & \hexaddress(8F83 8000) \\\hline
\end{tabular}
